Evolution of SASyLF 2008-2021

SASyLF was released in 2008 and used as a proof assistant in courses at several universities. It proved itself useful and has continued to be used, and each iteration of use has encouraged further development: fixing bugs and adding enhancements. This paper describes how SASyLF was developed while keeping true to its purpose. Most notable are making substitutions explicit, support of "and" and "or," support for mutual and lexicographic induction, and IDE support.

==> eptcsdata.tex <==
\providecommand{\firstpage}{87}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2021 (ThEdu'21)\\
EPTCS 354, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.354.7}{10.4204/EPTCS.354.7}}
\pdfoutput=1

